Characterizing Soft-Error Resiliency in Arm's Ethos-U55 Embedded Machine Learning Accelerator

As Neural Processing Units (NPU) or accelerators are increasingly deployed in a variety of applications including safety critical applications such as autonomous vehicle, and medical imaging, it is critical to understand the fault-tolerance nature of the NPUs. We present a reliability study of Arm's Ethos-U55, an important industrial-scale NPU being utilised in embedded and IoT applications. We perform large scale RTL-level fault injections to characterize Ethos-U55 against the Automotive Safety Integrity Level D (ASIL-D) resiliency standard commonly used for safety-critical applications such as autonomous vehicles. We show that, under soft errors, all four configurations of the NPU fall short of the required level of resiliency for a variety of neural networks running on the NPU. We show that it is possible to meet the ASIL-D level resiliency without resorting to conventional strategies like Dual Core Lock Step (DCLS) that has an area overhead of 100%. We achieve so through selective protection, where hardware structures are selectively protected (e.g., duplicated, hardened) based on their sensitivity to soft errors and their silicon areas. To identify the optimal configuration that minimizes the area overhead while meeting the ASIL-D standard, the main challenge is the large search space associated with the time-consuming RTL simulation. To address this challenge, we present a statistical analysis tool that is validated against Arm silicon and that allows us to quickly navigate hundreds of billions of fault sites without exhaustive RTL fault injections. We show that by carefully duplicating a small fraction of the functional blocks and hardening the Flops in other blocks meets the ASIL-D safety standard while introducing an area overhead of only 38%.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> det.tex <==
\section{Selective Detection Strategies}

We briefly talk about the various soft-error mitigation techniques available, along with the cost associated with them. We show how our $SDC_{NPU}$ formulation can be used to estimate the NPU resiliency when mitigation techniques are applied to the NPU.


\begin{scriptsize}
	\begin{table}[h!]
		\centering
		\caption{Available resilience techniques: sdc improvements and cost as a standalone solution}
		\label{table:formatting}
		\resizebox{\columnwidth}{!}{%
		\begin{tabular}{|l|l|l|l|l|}
			\hline
			\textbf{Technique} & \textbf{Area Cost} & \textbf{Power Cost} & \textbf{Prevents Logic Faults} & \textbf{SDC Improvement}\\
			\hline
			\hline
			Dual Modular Redundancy      & 100\%     &            & Yes                   & 100\%           \\ \hline
			DICE                         & 70\%      & 20\%       & No                    & 75\%            \\ \hline
			Quatro                       & 157\%     & -19\%      & No                    & 98\%            \\ \hline
			Heavy Ion Tolerant           &           &            &                       &                 \\ \hline
			TDFF~\cite{knudsen2006area}  &           &            &                       &                 \\ \hline
			DF-DICE~\cite{naseer2006df}  &           &            &                       &                 \\ \hline
			DURTPF~\cite{yan2019single}  &           &            &                       &                 \\ \hline
			SET Tolerant Power Optimized &           &            &                       &                 \\ \hline
  \end{tabular}
}
\end{table}
\end{scriptsize}

\subsection{Detection Strategies}
In this section, we look at the various hardware techniques proposed in the literature to reduce the SDC. We also compare the different strategies based on the overheads associated with them in terms of area, power, delay etc. 

\subsubsection{Modular Redundancy}
\paragraph{SDC Reduction}

\paragraph{Area Overhead}

\paragraph{Power Overhead}

\subsubsection{Flop Hardening}
\paragraph{Dual Interlocked Storage Cell.} DICE \cite{calin1996upset}. It is good for older technologies and not new ones\cite{amusan2008single,loveless2011neutron}.

\paragraph{Quatro.} Proposed in \cite{jahinuzzaman2009soft}

\paragraph{Heavy Ion Tolerant.}

\paragraph{SET Tolerant.} \cite{knudsen2006area,naseer2006df,yan2019single}

\paragraph{SET Tolerant Power Optimized.} \cite{jahinuzzaman2010tspc, jahinuzzaman2009soft,gupta2019soft}

\paragraph{SDC Reduction}

\paragraph{Area Overhead}

\paragraph{Power Overhead}


==> setup.tex <==
\section{Experimental Setup}

We describe our experimental setup and the ip used in this section and the breakdown of the workflow employed to obtain the data required for the Pareto-optimal configuration.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{scriptsize}
	\begin{table}[h!]
 
		\centering
		\caption{Available resilience techniques: sdc improvements and cost as a standalone solution}
		\label{table:schemes}
		\resizebox{\columnwidth}{!}{%
			\begin{tabular}{ccccc}
				%\hline
                    \toprule[0.15em]
				\textbf{Technique} & \textbf{Area Cost} & \textbf{Prevents Logic Faults} & \textbf{SDC Improvement}\\
				\midrule[0.05em]
				%\hline
				%\hline
				Dual Modular Redundancy      & 100\%              & Yes                   & 100\%           \\ %\hline
				DICE                         & 70\%             & No                    & 75\%            \\ %\hline
				Quatro                       & 157\%         & No                    & 98\%            \\ %\hline
				%Heavy Ion Tolerant           &                    &                       &                 \\ \hline
				%TDFF~\cite{knudsen2006area}  &           &            &                       &                 \\ \hline
				DF-DICE~\cite{naseer2006df}  &101.5\%                  &Yes                       &75\%                 \\ %\hline
				DURTPF~\cite{yan2019single}  & 210\%                  &Yes                       &95\%                 \\ %\hline
				TSPC-DICE~\cite{jahinuzzaman2010tspc} &46.05\%                    &Yes                       &75\%                 \\ %\hline
			\end{tabular}
		}
	\end{table}
\end{scriptsize}


\subsection{Reliability Evaluation}
\subsubsection{Baseline}
\label{sec:setup:baseline}
We use RTL fault injection to obtain ground truth resiliency data. We use Synopsys Z01X\texttrademark~\cite{z01x}, which is an industrial-scale RTL fault injection tool, to pick hardware fault sites represented as \mbox{$<\mathbf{Cycle, FF, BP}>$}.

For a single run, the tool picks a single fault-site and performs the RTL simulation that runs the application to the end. For each application, we inject over 330K faults into the Arms Ethos U55 RTL and run the RTL simulations. This ensures that the ground truth resiliency data has less than 1\% of error margin with a 99\% confidence interval per application.

Table~\ref{tbl:prob} lists the application we use to evaluate the reliability of Arms Ethos U55. We choose two different networks for the Classification task, CifarNet~\cite{hosang2015taking} and ResNet-18~\cite{he2016deep}, to vary the size of the application running on the NPU. We also carry out a fault injection campaign while running Wav2Letter~\cite{collobert2016wav2letter}, a Automatic Speech Recognition (ASR) network by Meta. We were not able to run popular networks for Object Detection tasks as Ethos U55 currently does not support such networks~\cite{mlzoo}.

\subsubsection{Resilient Configurations}
We utilize Equ~\ref{eq:sdcnpu_block_samp} to quantify the resiliency of a soft-error resilient configuration. Each functional block can employ any of the available schemes mentioned in Table~\ref{table:schemes}, giving us a total of $6^8 = 1679616$ configurations. Once a scheme is chosen for a block, SDC contribution of the block is adjusted as per the SDC improvement of the particular scheme mentioned in Table~\ref{table:schemes}.

\subsubsection{Estimating Logic Fault Contribution}
\label{sec:logic_est}
The combinational logic Soft Error Rate ($SER_{Comb}$) can be pprecisely calculated using TIDEST~\cite{gill2009comparison} methdology. This methodology has been validated with beam experiments, and has been used to calculate $SER_{Comb}$ for representative logic circuits at advanced technology nodes~\cite{seifert2012soft}. However, the application of TIDEST methodology to estimate $SER_{Comb}$ at the functional block or chip level requires the execution of exhaustive circuit-level simulations for the entire block or chip. This is not feasible due to runtime limitations and convergence issues in SPICE simulations. Despite utilizing modern-day clusters, it has been observed that even estimating the error rate of a single combinational node can be a time-consuming process, taking up to several hours.

We use an alternate methodology described by Gill et al.~\cite{gill2009comparison} to determine an upper bound on the $SER_{Comb}$ at the functional block and eventually NPU level. THe formulation describes $SER_{Comb}$ as a percentage of nominal latch $SER$ and is calculated as:

\begin{equation}
	\begin{aligned}
		& \frac{\mathrm{SER}_{\text {comb }}}{\mathrm{SER}_{\text {Latch }}}\% \approx \mathrm{LD}_{\text {comb }} * freq * \\
		& *\left(FOM *\left\{\begin{array}{l}
			\frac{\left(\text { Fanin }^{<\mathrm{d}>+1}-1\right)}{\left(\text { Fanin-1}\right)} ; \text { Fanin }>1 \\
			<\mathrm{d}>\text {; Fanin }=1
		\end{array}\right)\right. \\
		&
		\label{eq:ser_comb}
	\end{aligned}
\end{equation}

where Figure of Merit (FOM) is a technology and frequency dependent parameter. 		

\todo{A table describing all the parameters for calculating above equation}

\subsection{Area Evaluation}
We use Synopsys Design Compiler with the TSMC 16nm library to obtain the area numbers for the Arm Ethos-U55 base configurations of MAC-32, MAC-64, MAC-128 and MAC-256. We estimate the area of a configuration by adding the area cost (in Table~\ref{table:schemes}) to the baseline area of each functional block..  
%\paragraph{\textbf{Power Evaluation}}

%\subsection{Validation Setup}
%This section puts forward the description of our validation setup, including details such as the IP we worked with, tools used for fault injection, workloads etc.

%\subsection{Validation Results}
%We compare the ground truth results obtained from fault injection in the IP, with the numbers obtained from our proposed framework on aspects like the final set of blocks chosen for duplication, reliability numbers etc. 

==> uses.tex <==
\begin{abstract}
As Neural Processing Units (NPU) or accelerators are increasingly deployed in a variety of applications including safety critical applications such as autonomous vehicle, and medical imaging, it is critical to understand the fault-tolerance nature of the NPUs.
We present a reliability study of Arm's Ethos-U55, an important industrial-scale NPU being utilised in embedded and IoT applications. 

We perform large scale RTL-level fault injections to find out if Ethos-U55 meet the highest resiliency standards for applications such as autonomous vehicles. We show that all the four configurations of the NPU, fall short of the required level of resiliency for a variety of neural networks running on the NPU. 
%We also show that the resiliency of the NPU varies drastically with parameters such as configuration size, applications and technology node.
 
We find configurations of Ethos-U55 that meets the resiliency requirements by utilising existing soft-error mitigation and detection strategies. We ensure that the optimal configuration search is constrained by the area overhead as Ethos-U55 is used in embedded and IoT settings. We show that it is possible to meet the ASIL-D level resiliency requirements for the Ethos-U55 without resorting to strategies like Dual Core Lock Step (DCLS) that has an area overhead of roughly 100\%. We make use of the varying level of resiliency within the various functional block in Ethos-U55 to achieve required resiliency levels by duplicating just 30\% of the functional blocks.
%The aim of this work is to solve the problem of meeting stringent reliability requirements under area constraints. One of the big roadblocks to carrying out such studies is to characterize the reliability of different components of the IP in a feasible manner. We show that methods like exhaustive fault injections can take months to finish for different applications. We also showcase that the design space can be infinitely large for modern-day IPs and hence there is a tradeoff in the granularity level of characterization of the hardware components. We put forward a formulation for quantifying the reliability of the entire chip by characterizing the functional blocks in the IP with hardware-level fault injections. We use this formulation to study the impact of different detection strategies in terms of their benefits on the overall reliability and the associated power, area, and performance overheads. We put forward resiliency characterization of the functional blocks, which can help in the design of future IPs for similar applications.
\end{abstract}
